Local Explanations via Necessity and Sufficiency: Unifying Theory and Practice

Necessity and sufficiency are the building blocks of all successful explanations. Yet despite their importance, these notions have been conceptually underdeveloped and inconsistently applied in explainable artificial intelligence (XAI), a fast-growing research area that is so far lacking in firm theoretical foundations. Building on work in logic, probability, and causality, we establish the central role of necessity and sufficiency in XAI, unifying seemingly disparate methods in a single formal framework. We provide a sound and complete algorithm for computing explanatory factors with respect to a given context, and demonstrate its flexibility and competitive performance against state of the art alternatives on various tasks.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> sections/framework.tex <==
As discussed in the previous section, there have been distinct prior works on defining necessity and sufficiency in terms of input features (\cite{mothilal2020_unif, pertinent_negatives}), feature predicates (\cite{Ribeiro2018}), and causal interventions (\cite{tian2000probabilities,halpern2016actual}).
Here, we attempt to unify these works in a common framework. 
Our framework defines sufficiency and necessity in terms of conditional probabilities over a distribution of counterfactuals.
By allowing counterfactuals to be tagged with the interventions that led to them, we are able to establish sufficient and necessity of Anchors style feature predicates as well as~\cite{tian2000probabilities} style causal interventions in the same framework.
%Our framework is very similar to that of Anchors~(\cite{Ribeiro2018}) with certain tweaks allows us to offer a common definition of necessity and sufficiency to causal interventions and Anchors style predicates. 
%by introducing \emph{augmented counterfactuals} an abstract notion of \emph{factors} (defined below) whose necessity and sufficiency is established.

We focus on identifying necessary and sufficient factors for the prediction on an individual input $\inporig$. We restrict our attention to the binary classification setting, with $\modelfn: \inputspace \mapsto \{0,1\}$; extensions to regression may be implemented through a binary partition of continuous outcomes.

\stitle{Augmented Counterfactuals} Similar to most explainability methods, the starting point of our framework is a space of counterfactual inputs. These are meant to be alternatives to the protagonist input $\inporig$ that are examined for establishing sufficiency and necessity of various factors. They may be drawn from the training distribution or synthetically constructed by perturbing $\inp$.

We allow counterfactuals to be optionally tagged with  auxiliary information. Thus, a counterfactual input is $(\inp,\aug) \in \inputspace \times \augspace$ where $\augspace$ is the space of augmentations. The augmented features ($\aug$) may represent metadata associated with the counterfactual, for instance, demographic features that are otherwise not present in the input ($\inp$) seen by the model. They may also represent provenance information, for instance, specifying which intervention created the counterfactual (more on this in Section ??). The purpose of the augmentation is so that we can also consider sufficiency and necessity of factors based on such auxiliary information as well. In settings, where we are only interested in factors pertaining to the model input $\inp$, the augmentation $\aug$ may be empty. 

We assume a distribution  $\distrcf$ over a space of augmented counterfactuals corresponding to the protagonist input $\inporig$.
We use $Z, Z_1, \ldots$ for random variables distributed according to $\distrcf$.
Finally, we extend the model function to augmented inputs $(\inp, \aug)$ by defining $\modelfn((\inp, \aug)) = \modelfn(\inp)$.

\stitle{Factors} These are properties of interest associated with counterfactual inputs, whose necessity and sufficiency we wish to establish.
Formally, a factor $\factor$ is a predicate over a counterfactual $(\inp, \aug) \in \supp(\distrcf)$.
For instance, if $\inp$ is an input to a credit lending model, and $\aug$ represents demographic attributes, a factor may be the predicate $\inp[\mathsf{``income"}] \geq 500k~\wedge~\aug[\mathsf{``gender"}] = \mathsf{``female"}$ (checking if the example corresponds to a high income female). 
For another example, consider a case where the augmentation $\aug$ (in the counterfactual $(\inp, \aug)$) represents the set of features of the protagonist input $\inporig$ that were intervened upon to create $\inp$. Here, a factor may be the predicate $\{``income"\} \subseteq \aug$ (checking if $\mathsf{``income"}$ was intervened upon to create the counterfactual). We assume a finite space of factors $\factorspace$.

%A factor may simply be a predicate over input features (e.g., $\inp[\mathsf{fico}] \geq 700$) in which case $P(C=1~\vert~x)$ is 1 for all $x$ where the predicate is true, and 0 otherwise. A factor may also be probabilistic. For instance, for a model predicting readmission risk of patients, a factor may be “cardiovascular risk” defined by $P(\mathsf{cardiovascular~risk}~\vert~\mathsf{patient})$. Factors may also be properties associated with metadata or provenance of the counterfactuals, for instance, the interventions that led to the counterfactuals.
%We assume a finite space of factors $\factorspace$ and also assume that all factors are conditionally independent of each other given the input, i.e., $P(\factor_1~\wedge~\factor_2~\vert~\inp) = P(\factor_1~\vert~\inp) \star P(\factor_1~\vert~\inp)$.

\stitle{Partial order} When multiple sufficient factors are identified, we may prefer some factors over others. For instance, the sufficient factor $\inp[\mathsf{fico}] \geq 700$ would be preferred over $\inp[\mathsf{fico}] \geq 700 \land \inp[\mathsf{income}] \geq 10000$. 
Similarly, when two different interventions are identified as sufficient for a certain outcome, we may prefer the one with lower cost. 
We formalize this by allowing a partial order $\preceq$ over factors. 
When $\factor_1 \preceq \factor_2$, $\factor_1$ may be preferred over $\factor_2$.

One definition of $\factor_1 \preceq \factor_2$ is $\factor_1 \implies \factor_2$.
However, we emphasize that this is not the only definition.
In Section ??, we show many other definitions, and argue how the choice of partial order is a useful knob in identifying sufficient factors for different applications.

We are now ready to formally specify our framework.
\begin{defn}[Framework]\label{def:framework}
Our framework for identifying necessary and sufficient factors for given input $\inporig$ is specified by the tuple $\langle \modelfn, \distrcf, \factorspace, \preceq \rangle$ where $\modelfn$ is the model function, $\distrcf$ is the (augmented) counterfactual distribution for input $\inporig$, $\factorspace$ is the space of potential factors, and $\preceq$ is a partial order over factors.
\end{defn}

\subsection{Necessity and Sufficiency}
In tune with classical logic, we define a factor $\factor$ to be \emph{sufficient} for an outcome y if the factor implies the outcome, i.e., $\factor(Z) \implies \modelfn(Z) = y$, and \emph{necessary} for an outcome $y$ if the outcome implies the factor, i.e., $\modelfn(Z) = y \implies \factor(Z)$. Since, a factor may only partially imply an outcome, we extend these notions to their probabilistic counterparts.

\begin{defn}[Probability of Sufficiency]\label{def:probsuff}
The probability of sufficiency of a factor $\factor$ for an outcome y, denoted by $\probsuff(\factor, y)$, is $\prob(\modelfn(Z) = y~\vert~\factor(Z)]$ where $Z\sim\distrcf$
\end{defn}

\begin{defn}[Probability of Necessity]\label{def:probnecc}
The probability of necessity of a factor $\factor$ for an outcome y, denoted by $\probnecc(\factor, y)$ is $\prob(\factor(Z)~\vert~\modelfn(Z) = y)$ where $Z\sim\distrcf$
\end{defn}

The definitions of probability of sufficient and necessity can be naturally extended to a set of factors $\factorset = \{\factor_1, \ldots, \factor_k\}$ by defining $\probnecc(\factorset, y) \Coloneqq \prob(\bigvee_{i=1}^{k}\factor_i(Z)~\vert~\modelfn(Z) = y)$,
and $\probsuff(\factorset, y) \Coloneqq \prob(\modelfn(Z) = y~\vert~\bigvee_{i=1}^{k}\factor_i(Z))$.

We call a factor \emph{perfectly} sufficient (necessary) for an outcome if its probability of sufficiency (necessity) is 1.
We then prove a simple proposition stating that perfectly sufficient and necessary factors are unique.
\begin{prop}\label{prop:suffnecc}
If a factor $\factor$ is perfectly sufficient and necessary for an outcome $y$ then any other factor $\factor' \in \factorspace$ that is also perfectly sufficient and a necessary for $y$ must be logically equivalent to $\factor'$ over $\distrcf$, i.e., $\forall (\inp, \aug) \in \supp(\distrcf): \factor((\inp, \aug)) = \factor'((\inp, \aug))$.
\end{prop}
While the above proposition seems obviously true
for our definitions, in Section ?? we show that it does not hold for the definitions of sufficiency and necessity proposed in~\cite{tian2000probabilities}.


\begin{remark}
Our framework is inspired by that of Anchors~\cite{Ribeiro2018}, and indeed our definition of probability of sufficiency is equivalent the definition of ``precision'' of Anchors.
Our probability of necessity is slightly different from the definition of ``coverage'' of Anchors, in that, we are interested in the coverage of a factor over counterfactuals that achieve a certain outcome as opposed to everywhere.
The primary novelty of our framework lies in extending the idea of Anchors to a broader notion of factors that may go beyond predicates on feature values, and may pertain to the provenance of the counteractuals, for instance, the interventions that led to them.
\end{remark}

\begin{remark}
The probability of sufficiency and necessity of a factor $\factor$ for an outcome $y$ can be likened to the ``precision'' (positive predictive value) and ``recall'' (true positive rate) of a (hypothetical) classifier that predicts whether $F(Z) = y$ based on whether $C(Z)$ holds.
By examining the confusion matrix of this classifier, one can define many related quantities, for instance, negative predictive value ($\prob(F(Z) \neq y~\vert~\neg\factor(Z))$), true negative rate ($\prob(\neg\factor(Z)~\vert~F(Z) \neq y)$), and so on. 
These quantities may also be of interest in certain applications.
In this work, we limit ourselves to just probability of sufficiency and necessity as they suffice for the applications we consider.
\end{remark}

\subsection{Identifying Minimal Sufficient Factors}
We now discuss an abstract procedure for identifying all \emph{minimal} sufficient factors for an outcome $y$ with probability of sufficiency above a given threshold $\tau$.
Here, a factor $\factor$ is considered minimal if there does not exist a factor $\factor'$ such that $\factor' \preceq \factor$ and $\factor'$ also has a probability of sufficiency of at least $\tau$.

Our procedure for a given framework $\langle \modelfn, \distrcf, \factorspace, \preceq \rangle$ is outlined in Algorithm~\ref{alg:main}; see the method \textsf{minimalSufficientFactors}.
The key idea is to topological sort the space of factors w.r.t. $\preceq$, and iterate over them.
In each iteration, we select a factor $\factor$ if
no factor $\factor'$ such that $\factor' \preceq \factor$ has previously been selected, and $\factor$ has a probability of sufficiency of at least $\tau$.

The probability of sufficiency of a factor $\factor$ for an outcome $y$ is computed (see the method \textsf{probSufficiency})
by estimating $\expect[1_{\modelfn(Z_\factor) = y}]$ where $Z_\factor\sim \distrcf(\cdot~\vert~\factor)$.
It is easy to see that this formulation is equivalent to Definition~\ref{def:probsuff}.
It is helpful in settings where one can directly sample from $\distrcf(\cdot~\vert~\factor)$, which happens to be case for all our applications.

Finally, we report the cumulative probability of necessity of the returned set $\factorset$ of minimal factors (see the method \textsf{probNecessity}).
The probability of necessity gives a sense of what fraction of the counterfactual where the outcome is y are covered by the factors in $\factorset$. 
Since, a minimal factor $\factor$ stands for all factors $\factor'$ such that $\factor \preceq \factor'$, in reporting probability of necessity, we expand $\factorset$ to its upward closure.

\stitle{Correctness guarantee}
To state the correctness guarantee for our procedure, we first formalize the notion of minimality.

\begin{defn}[$\tau$-minimality]\label{defn:minimality}
A factor $\factor$ is $\tau$-minimal for an outcome $y$ if $\probsuff(\factor, y) \geq \tau$ and $\neg \exists \factor' \in \factorspace: (\factor'\preceq\factor~\wedge~\probsuff(\factor',y)\geq\tau$).
\end{defn}
We now state our correctness theorem.
\begin{theorem}\label{thm:correctness}
If $\factorset$ is the set of factors returned by \textsf{minimalSufficientFactors} then for any factor $\factor \in \factorspace$, $\factor$ is $\tau$-minimal if and only if $\factor\in\factorset$.
\end{theorem}

%\begin{defn}[coverage]\label{defn:minimality}
%The space of factors $\factorspace$ covers the counterfactual distribution $\distrcf$ if for each $(\inp, \aug) \in \supp(\distrcf)$, there exists a factor $\factor \in \factorspace$ such that $\factor((\inp, \aug))$ holds.
%\end{defn}

TODOs: (a) caveat theorem with estimation error.

\begin{algorithm}[!ht]
  \caption{Identifying Minimal Sufficient Factors}\label{alg:main}
 \begin{algorithmic}
  \STATE {\bfseries Framework:} $\langle \modelfn, \distrcf, \factorspace, \preceq \rangle$
  \STATE
  \STATE {\bfseries function} {probSufficiency}{($\factor$, $y$)}
      \begin{ALC@g}
        \STATE {\bfseries sample} $\distrfactorhat ::= \{(\inp_1,\aug_1), \ldots, (\inp_n, \aug_n)\} \sim  \distrcf(\cdot~\vert~\factor)$
        \STATE n\_fac\_out = $\sumfn(\{\mathds{1}~\vert~ (\inp_i, \aug_i) \in \distrfactorhat\mbox{ and } \modelfn(\inp_i)=y\})$
        \STATE {\bfseries return} n\_fac\_out~/~n
      \end{ALC@g}
  \STATE
    
  \STATE {\bfseries function} {probNecessity}{($\factorset  = \{\factor_1, \ldots, \factor_k\}$, $y$, upward\_closure)}
    \begin{ALC@g}
      \IF{upward\_closure}
          \STATE $\factorset  =  \{\factor~\vert~\factor \in \factorspace \mbox{ and } \exists~\factor' \in \factorset: \factor' \preceq \factor\}$
      \ENDIF            
      \STATE {\bfseries sample} $\distrfactorhat ::= \{(\inp_1,\aug_1), \ldots, (\inp_n, \aug_n)\} \sim  \distrcf$
      \STATE n\_fac\_out = $\sumfn(\{(\mathds{1}~\vert~\cfinp \in \distrhat\mbox{ and } \modelfn(\cfinp)=y\})$
      \STATE n\_out = $\sumfn(\{\mathds{1}~\vert~ \cfinp \in \distrhat \mbox{ and } \modelfn(\cfinp)=y\})$
      \STATE {\bfseries return} n\_fac\_out~/~n\_out
    \end{ALC@g}
  \STATE

  \STATE {\bfseries function} {minimalSufficientFactors}{($y$, $\tau$)}
    \begin{ALC@g}
      \STATE sorted\_factors = $\toposortfn(\factorspace, \preceq)$
      \STATE cands = []
      \FOR {$\factor$ in sorted\_factors}
        \IF {$\exists (\factor', \_) \in\mbox{ cands }: \factor'\preceq\factor$}
          \STATE {\bfseries continue}
        \ENDIF
        \STATE ps = probSufficiency($\factor$, $y$)
        \IF{ps >= $\tau$}
          \STATE cands.append(($\factor$, ps))
        \ENDIF
        \ENDFOR
      \STATE cum\_pn = probNecessity($\{\factor~\vert~(\factor, \_) \in \mbox{cands}\}$, y, True) 
      \STATE {\bfseries return} cands, cum\_pn
    \end{ALC@g}
 \end{algorithmic}
\end{algorithm}

\footnote{This is identical to the formulation used by \citep{Ribeiro2018} to define sufficiency of Anchors.}

==> sections/theory.tex <==
% We highlight three key properties of successful explanations, drawing on the pragmatic tradition in philosophy and social science \citep{Kahneman1986, Woodward2003a, Blaauw2013, Floridi2019, Miller_2019}: 

% \begin{enumerate}[noitemsep,topsep=0pt]
%     \item \emph{Causal}. Explanations help agents answer ``what if" questions (henceforth $w$-questions) about how the target system(s) would respond to interventions.
%     \item \emph{Contrastive}. Explanations evaluate their target relative to some baseline expectation(s). 
%     \item \emph{Interactive}. Explanations are iterative and dynamic; they are a process, not a product.
% \end{enumerate}

The dominant XAI methods in use today fall short in several respects. Take SHAP \citep{lundberg_lee_2017}, the aforementioned local linear approximator. Several authors (including the developers themselves) have acknowledged that the algorithm's default settings -- which fix baseline expectations at the empirical mean $\phi_0 = n^{-1} \sum_{i=1}^n f(\bm{x}_i)$, and sample subvectors $\bm{X}^R$ from their marginal distribution -- are limiting, to say the least. Such restrictions prevent users from asking perfectly sensible questions, like why they received an average credit score instead of a better-than-average one, or conditioning on immutable features such as race to ensure they receive zero attribution. Recent work has sought to expand the scope of reference distributions for $\bm{X}^R$ \citep{Aas2019, heskes2020} and allow for more generic contrasts \citep{Ramon2020}, but such changes threaten to undermine the uniqueness result that attracts many practitioners to Shapley values in the first place \citep{Sundararajan2019}.

Counterfactuals are more flexible, identifying real or synthetic datapoints that differ from the explanans in specific ways. However, they face several challenges of their own \citep{barocas2020}. Most important for our purposes is the question of how wide a range of counterfactuals to provide. The optimization problem expressed by Eq.~\ref{eq:cf} suggests that just a single sample would suffice. This vastly overestimates the certainty with which such a datapoint is generated. Can we really be sure that $\bm{x}^*$ is to be preferred to some other counterfactual $\bm{x}'$ just because the former is marginally closer in feature space to the input $\bm{x}_i$? It is not obvious that very small distances should be taken seriously when there are so many potential sources of noise -- in the measurements themselves, in the finite training data, and in whatever approximations were required to efficiently compute candidate counterfactuals. That is why some authors prefer to sample a large, diverse coalition of counterfactuals \citet{mothilal2020_dice}, so that users can survey the various paths through which a prediction can change. Yet this approach raises new problems of intelligibility. How should an agent make sense of a counterfactual subspace with dozens or hundreds of samples within a tolerable distance of $\bm{x}_i$? How should she prioritize among different counterfactuals or integrate this information into a high-level summary?

Our solution is to go back to feature attribution methods with a renewed focus on necessity, sufficiency, and contrastive reasoning. We begin with some definitions. Input features and model predictions together constitute the endogenous variables of $\mathcal{M}$, $\bm{V} = \{\bm{X}, Y = f(\bm{X})\}$. We restrict attention here to the classification setting, with $Y \in \{0,1\}$; extensions to regression may be implemented through a binary partition of continuous outcomes.

\begin{defn}[Input space] \label{def:inp_space}
    The input point $\bm{v}_i = (\bm{x}_i, y_i)$ is drawn from an associated input space, $\mathcal{I} := P(\bm{V}|\bm{v}_i)$. 
\end{defn}

This, of course, is a degenerate distribution. We could conceivably expand the space to $\mathcal{M}(\bm{U}|\bm{v}_i)$ at some loss to locality. (More on this below.) 

\begin{defn}[Reference space] \label{def:ref_space}
    Let $Q \subseteq [d]$ be a (possibly empty) subset of features a user wants to hold (approximately) fixed in constructing a contrast class. Reference points $\tilde{\bm{v}}$ are drawn from an associated reference space, $\mathcal{R} := \mathcal{M}(\bm{U}|\bm{x}^Q, \tilde{y})$, where $\tilde{y} \neq y_i$. 
\end{defn}


% Let $\{S_k\}_{k=1}^{2^d}$ denote the powerset of $[d]$, and let $\tau$ be some decision threshold, conventionally fixed at $0.5$. We want to measure the extent to which intervening on particular feature subsets tends to alter expected outcomes. To do so, we define two indicator variables. $Z^{\mathcal{I}}$ records the effects of replacing input subvectors with reference subvectors. The $k^{\text{th}}$ entry is given by:

% \begin{align*}
%     z_k^{\mathcal{I}} = \mathds{1} [P_{\mathcal{I}}(\tilde{y} | do(\tilde{\bm{x}}^{S_k})) \geq \tau].
% \end{align*}

% $Z^{\mathcal{R}}$ records the effects of replacing reference subvectors with input subvectors. The $k^{\text{th}}$ entry is given by:

% \begin{align*}
%     z_k^{\mathcal{R}} = \mathds{1} [P_{\mathcal{R}}(y_i | do(\bm{x}_i^{S_k})) \geq \tau].
% \end{align*}

% These variables allow us to define weak notions of causal necessity and sufficiency.

% \begin{defn}[Causal necessity (weak)] \label{def:cn_weak}
%     Feature subset $S_k$ is a weakly necessary cause of $y_i$ iff $z_k^{\mathcal{I}} = 1$.
% \end{defn}

% \begin{defn}[Causal sufficiency (weak)] \label{def:cs_weak}
%     Feature subset $S_k$ is a weakly sufficient cause of $y_i$ iff $z_k^{\mathcal{R}} = 1$.
% \end{defn}

% These definitions are weak in the sense that they restrict the range of permissible interventions to just a single regime. We may strengthen them by demanding comparable effects no matter what other interventions are present. Let $Z^{\mathcal{I}}_{S}$ denote all $z_k^{\mathcal{I}}$ such that $S_k \supseteq S$, and define $Z^{\mathcal{R}}_{S}$ analogously. 

% If $|S|$ is the number of elements in $S$, then the cardinality of $Z^{\mathcal{I}}_{S}$ is given by $m = ( \genfrac{}{}{0pt}{}{2^d}{|S|} )$. Strong notions of causal necessity and sufficiency can now be defined as follows.

% \begin{defn}[Causal necessity (strong)] \label{def:cn_strong}
%     The probability that feature subset $S$ is a strongly necessary cause of $y_i$ is $P_{\mathcal{I}}(Z_k^{\mathcal{I}})$.
% \end{defn}

% \begin{defn}[Causal sufficiency (strong)] \label{def:cs_strong2}
%     The probability that feature subset $S$ is a strongly sufficient cause of $y_i$ is $P_{\mathcal{R}}(Z^{\mathcal{R}}_{S})$.
% \end{defn}

% We consider two possible types of interventions: those that set variables to their input values, e.g. $do(\bm{x}_i^S)$; and those that set variables to their reference values, e.g. $do(\tilde{\bm{x}}^S)$. 

Measures of necessity and sufficiency can now be defined for any given feature subset. We begin with weak measures, which closely track those of \citet{tian2000probabilities} and \citet{Pearl2000}. However, we extend their results to arbitrary dimensions and continuous features, while also modifying their (implicit) notion of a reference space. 

\begin{defn}[Causal necessity (weak)] \label{def:nec}
    The probability that feature subset $\bm{x}_i^S$ is a weakly necessary cause of $y_i$ is:
    \begin{align*}
        \texttt{nec}(S) := P_{\mathcal{I}}(\tilde{y}|do(\tilde{\bm{x}}^S)).
    \end{align*}
    \texttt{nec} measures the extent to which intervening to replace input values with reference values would likely change an outcome, with probability taken over the input space.  
\end{defn}

\begin{defn}[Causal sufficiency (weak)] \label{def:suf}
    The probability that feature subset $\bm{x}_i^S$ is a weakly sufficient cause of $y_i$ is:
    \begin{align*}
        \texttt{suf}(S) := P_{\mathcal{R}}(y_i|do(\bm{x}_i^S)).  
    \end{align*}
    \texttt{suf} measures the extent to which intervening to replace reference values with input values would likely preserve an outcome, with probability taken over the reference space.  
\end{defn}

Two problems arise with these definitions in continuous, multi-dimensional settings. First, they implicitly place a uniform prior on all possible interventions, which means we may trivially maximize both measures by setting $S = [d]$. We would instead like to encode the intuition that minimal interventions are preferable. Second, these definitions do not account for potential interaction effects. For instance, say that $\texttt{suf}(\{1\}) = \texttt{suf}(\{2\}) = 0.9$; however,  $\texttt{suf}(\{1,3\}) = 0.1$ and $\texttt{suf}(\{2,3\}) = 0.9$. In this case, we would like to favor $X_2$ over $X_1$, as the former is clearly more resilient to auxiliary perturbations. To resolve both issues, we propose the following measures.

\begin{defn}[Causal necessity (strong)] \label{def:NEC}
    The probability that feature subset $\bm{x}_i^S$ is a strongly necessary cause of $y_i$ is:
    \begin{align*}
        \texttt{NEC}(S) := \mathds{E}_{\mathcal{I}}[\texttt{nec}(S_k: S_k \supseteq S)].
    \end{align*}
    \texttt{NEC} measures the extent to which intervening to replace input values with reference values would likely change an outcome, even if other interventions are present. Expectation is taken over the input space.
\end{defn}

\begin{defn}[Causal sufficiency (strong)] \label{def:SUF}
    The probability that feature subset $\bm{x}_i^S$ is a strongly sufficient cause of $y_i$ is:
    \begin{align*}
        \texttt{SUF}(S) := \mathds{E}_{\mathcal{R}}[\texttt{suf}(S_k: S_k \supseteq S)].
    \end{align*}
    \texttt{SUF} measures the extent to which intervening to replace reference values with input values would likely preserve an outcome, even if other interventions are present. Expectation is taken over the reference space.
\end{defn}

% Together, these measures tell us both why an outcome was so and not otherwise. But the converse relationships are of explanatory interest as well. For instance, are there many other interventions that might have preserved or changed a given prediction? We label these notions causal sensitivity and specificity, by analogy with similar concepts in frequentist inference. 

% We presume that agents may rationally place variable weight on PN or PS depending on their analytical goals, but some combination of the two is typically desirable. One particular convex combination enjoys special properties:

% \begin{defn}[Probability of necessity and sufficiency] \label{def:pns}
%     The probability that feature subset $\bm{x}_i^S$ is a necessary and sufficient cause of $y_i$ is:
%     \begin{align*}
%         \text{PNS} := P(\bm{x}_i^S, y_i)\text{PN} + 
%         P(\tilde{\bm{x}}^S, \tilde{y})\text{PS}.  
%     \end{align*}
%     PNS measures the extent to which $\bm{X}^S$ determines outcomes one way or another.  
% \end{defn}

% There is an intriguing formal similarity between these measures and familiar machine learning performance metrics. Consider a confusion matrix with columns $y = 1, y = 0$ and rows $\hat{y} = 1, \hat{y} = 0$. The cells of this matrix, moving clockwise from the top left, correspond to true positives (TP), false positives (FP), true negatives (TN), and false negatives (FN). Now replace the columns with $y, y'$ and the rows with $do(x), do(x')$. Assume that the top row is computed with respect to the reference space, and the bottom with respect to the input space. Then NEC is analogous to the negative predictive value, i.e. TN/(TN + FN), and SUF to the positive predictive value, i.e. TP/(TP + FP).

% This immediately suggests alternative measures of causal influence, borrowed again from confusion matrix analysis. Translated into our setting, sensitivity and specificity -- given by TP/(TP + FN) and TN/(TN + FP), respectively -- acquire new interpretations, formalized below.

% \begin{defn}[Causal sensitivity (weak)] \label{def:sens}
%     Let $\beta$ denote a sufficiency threshold, such that we restrict attention to only those interventions $do(\bm{x}_i^S)$ such that $\texttt{SUF}(S) \geq \beta$. The weak causal sensitivity of $\bm{x}_i^S$ on $y_i$ is:
%     \begin{align*}
%         \texttt{sens(S)} := P_{\mathcal{R}}(do(\bm{x}_i^S)|y_i, \beta).
%     \end{align*}
%     \texttt{sens} measures the likelihood that a particular intervention $\beta$-preserves an outcome, given that some intervention does so.
% \end{defn}

% \begin{defn}[Causal specificity (weak)] \label{def:spec}
%     Let $\alpha$ denote a necessity threshold, such that we restrict attention to only those interventions $do(\tilde{\bm{x}}^S)$ such that $\texttt{NEC}(S) \geq \alpha$. The causal specificity of of $\bm{x}_i^S$ on $y_i$ is:
%     \begin{align*}
%         \texttt{spec(s)} := P_{\mathcal{I}}(do(\tilde{\bm{x}}^S)|\tilde{y}, \alpha).
%     \end{align*}
%     \texttt{spec} measures the likelihood that a particular intervention $\alpha$-changes an outcome, given that some intervention does so.
% \end{defn}

% \begin{defn}[Causal sensitivity (strong)] \label{def:SENS}
%     The strong causal sensitivity of $\bm{x}_i^S$ on $y_i$ is:
%     \begin{align*}
%         \texttt{SENS(S)} := \mathds{E}_{\mathcal{R}}[\texttt{sens}(S_k: S_k \supseteq S)].
%     \end{align*}
%     \texttt{SENS} measures the likelihood that a particular intervention $\beta$-preserves an outcome, given that some intervention does so, even if other interventions are present.
% \end{defn}

% \begin{defn}[Causal specificity (strong)] \label{def:SPEC}
%     The strong causal specificity of of $\bm{x}_i^S$ on $y_i$ is:
%     \begin{align*}
%         \texttt{SPEC(s)} := \mathds{E}_{\mathcal{I}}[\texttt{spec}(S_k: S_k \supseteq S)].
%     \end{align*}
%     \texttt{spec} measures the likelihood that a particular intervention $\alpha$-changes an outcome, given that some intervention does so, even if other interventions are present.
% \end{defn}

% Taken together, these four measures provide an exhaustive overview of the explanatory value of a feature subset for a target outcome. The first two measures factor into several existing XAI methods; the latter two, to the best of our knowledge, are novel.

Though rarely spelled out in formal detail, \texttt{nec} and \texttt{suf} can be shown to play a central role in feature attributions, counterfactuals, and rule lists. Because many methods presume feature independence, we will occasionally require the assumption of ignorability to state the subsequent propositions.

\begin{defn}[Ignorability] \label{def:ignorability}
    Feature subset $\bm{X}^S$ is ignorable for $Y$ in $\mathcal{M}$ iff $P(Y|do(\bm{x}^S)) = P(Y|\bm{x}^S)$ for all possible values of $\bm{X}^S$. 
\end{defn}

Following \citet{taly2020}, we rewrite Eq.~\ref{eq:val} in a more general form to acknowledge the variety of reference distributions available for $\bm{X}^R$:

\begin{equation} \label{eq:val2}
    v_{\mathcal{D}_R}(S) = \mathbb{E}_{\bm{X}^R \sim \mathcal{D}_R}[f(\bm{x}_i^S, \bm{X}^R)].
\end{equation}

We consider three possible values of $\mathcal{D}_R$: marginal $P(\bm{X}^R)$, as in \citep{lundberg_lee_2017}; conditional $P(\bm{X}^R|\bm{x}_i^S)$, as in \citep{Aas2019}; and interventional $P(\bm{X}^R|do(\bm{x}_i^S))$, as in \citep{heskes2020}. 

Let $\mathcal{R}' := \mathcal{M}(\bm{U})$ denote a modified reference space, sampled at random from (or simply equivalent to) the empirical dataset, and let $\texttt{suf}'$ denote the corresponding measure of causal sufficiency taken over this reference. 

\begin{prop} \label{prop:shap1}
    When $\mathcal{D}_R$ is the interventional distribution, $v_{\mathcal{D}_R}(S) = \texttt{suf}'(S)$.
\end{prop}
    
\begin{prop} \label{prop:shap2}
    When $\mathcal{D}_R$ is the marginal or conditional distribution and $\bm{X}^S$ is ignorable for $Y$, then $v_{\mathcal{D}_R}(S) = \texttt{suf}'(S)$.
\end{prop}

In other words, under any reference distribution, the Shapley value of an individual predictor is just its average marginal contribution to the causal sufficiency of a random feature subset.

For counterfactuals, we can rewrite the optimization target in terms of input and reference spaces. Let $\mathcal{I}' := \mathcal{M}(\bm{U}|\bm{v}_i)$ be an expanded (non-degenerate) input distribution with a mode at $\bm{v}_i$, and $\texttt{nec}'$ the corresponding measure of causal necessity taken over this space. 

\begin{prop} \label{prop:cf1}
    Let $cost(\bm{x}_i, \tilde{\bm{x}})$ be a monotonically decreasing function of $P_{\mathcal{I}'}(\tilde{\bm{x}})$, e.g. the negative log-likelihood. If all feature subsets $\bm{X}^S$ are ignorable for $Y$, then Eq.~\ref{eq:cf} is equivalent to:
    \begin{equation} \label{eq:cf2}
        \bm{x}^* = \argmax_{\tilde{x} \sim \mathcal{R}} ~P_{\mathcal{I}'}(\tilde{x}).
    \end{equation}
\end{prop}

When dependencies between predictors are present, as in \citep{karimi2020imperf}, then the optimization target shifts from a search over references to a search over interventions.

\begin{prop} \label{prop:cf2}
    If some feature subset $\bm{X}^S$ is not ignorable for $Y$, then the recourse objective is to compute the cost-minimizing intervention that exceeds a lower bound on causal necessity:
    \begin{equation}
    \begin{aligned}
        S^* = \argmin_{S \subseteq [d]} ~&cost(\bm{x}_i, do(\tilde{\bm{x}}^S)) \\
        \textrm{s.t.} ~&\texttt{nec}'(S) \geq \alpha,
    \end{aligned}
    \end{equation}
    where $\alpha$ denotes a decision threshold.
\end{prop}

Finally, we may reformulate precision and coverage -- the key concepts behind \citet{Ribeiro2018}'s anchors -- using $\mathcal{R}'$ and $\texttt{suf}'$, as above. 

\begin{prop} \label{prop:anchors}
    If anchors $A$ are ignorable for $Y$, then $\text{prec}(A) = \texttt{suf}'(A)$. Coverage is given by $P_{\mathcal{R}'}(A)$.
\end{prop}

These propositions clarify the similarities and differences between these XAI approaches, which rely on weak notions of necessity and sufficiency to varying degrees. Moreover, they allow us to quickly diagnose problematic elements of existing proposals, such as unmotivated modifications to the reference space and a narrow focus on weak concepts of necessity or sufficiency. By elevating the analysis to feature subsets and simultaneously optimizing for necessity and sufficiency, we can compute more general and satisfying explanations.


% Pragmatic epistemologists have long argued that explanations are best understood as answers to questions. Intuitively, the criteria above are intended to empower users to answer questions such as:

% \begin{itemize}[noitemsep,topsep=0pt]
%     \item Why did $f$ predict $\hat{y}_i$ as opposed to $\tilde{y}$ for $\bm{x}_i$?
%     \item Why did $f$ predict $\hat{y}_i$ as opposed to $\tilde{y}$ for $\bm{x}_i$, given $\bm{x}_i^S$?
%     \item Why did $f$ predict $\hat{y}_i$ as opposed to $\tilde{y}$ for $\bm{x}_i$, given $\bm{x_i}^S$ and certain constraints on $\bm{X}^R$?
% \end{itemize}



% \begin{defn}[Reference Class]
%     Let $S \subseteq [d]$ denote a (potentially empty) conditioning set with complement $R$. Let $\mathcal{D}_S$ be the space of permissible subvectors for the conditioning set, which reduces to the observed $\bm{x}_i^S$ in the limit. Alternatively, $\mathcal{D}_S$ may describe an $\epsilon$-ball around $\bm{x}_i^S$, with perhaps some additional restrictions on the joint distribution of variables $\{X_j\}_{j \in S}$. Let $\mathcal{D}_R$ be a distribution encoding probable variation in $\bm{X}^R$ as a function of $\bm{x}^S$. We say that sample $\tilde{\bm{x}}$ is an element of the reference class CF($\bm{x}_i$) iff: (i) $\tilde{\bm{x}}^S \sim \mathcal{D}_S$ and (ii) $\tilde{\bm{x}}^R \sim \mathcal{D}_R$. \blacksquare
% \end{defn}

% The primitive notions encoded in this definition are \emph{preservation} and \emph{change}, neither of which are absolutes but rather admit of degrees. The conditioning set $S$ may contain immutable features (e.g., race) or variables that can only move a small amount in a given period (e.g., savings). Preserving these values, or at least bounding their variance, is key. The free variables in $R$ may be completely unconstrained, or else depend on (some elements of) $S$. 



% Necessity: $p(\bm{x}_i^S | \hat{y}_i, \bm{x}_i^Q)$
% Sufficiency: $p(\hat{y}_i | do(\bm{x}_i^S), \bm{x}_i^Q)$
% We define a partition of the vector $\bm{x}_i$ into two disjoint sets $Q, R$, where $Q$ denotes a (potentially empty) set of conditioning events, e.g. immutable features, and $R$ denotes a set of free variables, which vary according to some reference distribution. The goal is to quantify the causal impact of some feature subset $S \subseteq R$, where the remaining features $R \backslash S$ may depend on $Q$ and/or $S$.



% \subsection{Definitions}
% \subsection{Sufficient causes} 
% Features that must be preserved in an input to preserve its prediction, e.g., preserving FICO=800 is sufficient to get the loan
% \subsection{Necessary causes} 
% Features that must be perturbed in an input to alter its prediction, e.g., perturbing income is sufficient to flip the outcome 
% \subsection{But for causes}
% bdas

% \subsection{Properties}


% \subsection{Multi-reference?}

% \subsection{Full causal knowledge and no causal knowledge}






% Why do we use interpretable machine learning tools in the first place? \citet{Watson_exp_game} offer three reasons: (1) to audit for potential bias; (2) to validate performance, guarding against unexpected errors; and (3) to discover underlying mechanisms of the data generating process. Another use case, with elements of (1) and (3) yet distinctly analyzed in the recourse setting, is (4) to recommend actions so as to alter predicted outcomes. These motivations may overlap at the edges but they represent distinct tasks based on different assumptions and requiring their own explanatory methodologies. This heterogeneity is largely ignored by current methods, which implicitly assume a sort of \emph{explanatory objectivism}. According to this view, the quality of an explanation is independent of its context.

% Decades of research in philosophy and social science has made such objectivism untenable \citep{Floridi2019, sep-pragmatism, Miller_2019}. If the view has any adherents today, perhaps it is because the alternative is often misconstrued as \emph{relativism}, an anything-goes slippery slope that inevitably leads to what \citet{Feyerabend1975} (approvingly) refers to as ``epistemological anarchism". This, however, is a false dichotomy. We reject the polar extremes of objectivism and relativism in favor of \emph{pragmatism}, which holds neither that there exists some single ideal explanation nor that all explanations are equally valid, but rather that various explanations may be more or less appropriate depending on who requests them and why. 

% Specifically, we consider According to \citet{Woodward2003a}, the goal of explanation is to help agents answer ``what if" questions (henceforth $w$-questions). 



% Let $\mathcal{D}_S$ be the space of permissible subvectors for the conditioning set, which reduces to the observed $\bm{x}_i^S$ in the limit. Alternatively, $\mathcal{D}_S$ may describe an $\epsilon$-ball around $\bm{x}_i^S$, with perhaps some further restrictions on the joint distribution of $\bm{X}^S$. Let $\mathcal{D}_{R|S}$ be a distribution encoding probable variation in $\bm{X}^R$ as a function of $\bm{x}^S$. Sample $\tilde{\bm{v}} = (\tilde{\bm{x}}^S, \tilde{\bm{x}}^R, \tilde{y})$ is a valid contrast for $\bm{v}_i$ iff (i) $\tilde{\bm{x}}^S \sim \mathcal{D}_S$, (ii) $\tilde{\bm{x}}^R \sim \mathcal{D}_{R|S}$, and (iii) $\tilde{y} \neq y_i$.

% The implicit contrast class for all SHAP explanations is the data centroid. This is because attributions only account for the discrepancy between $f(\bm{x}_i)$ and the empirical mean $\phi_0 = n^{-1} \sum_{i=1}^n f(\bm{x}_i)$. Moreover, SHAP samples subvectors $\bm{X}^R$ from their marginal distribution, thereby breaking any association with $\bm{x}_i^S$ and comparing each $x_{ij}$ to the mean of the corresponding variable $X_j$. Yet these might not be the relevant contrasts for a given agent, who may, for instance, want to know why she received an average credit score instead of a better-than-average one. Or perhaps she wants to compare her predictions only to those of others in a similar age and income bracket, effectively setting those feature attributions to zero. 
